DiffuScene: Denoising Diffusion Models for Generative Indoor Scene Synthesis

We present DiffuScene for indoor 3D scene synthesis based on a novel scene configuration denoising diffusion model. It generates 3D instance properties stored in an unordered object set and retrieves the most similar geometry for each object configuration, which is characterized as a concatenation of different attributes, including location, size, orientation, semantics, and geometry features. We introduce a diffusion network to synthesize a collection of 3D indoor objects by denoising a set of unordered object attributes. Unordered parametrization simplifies and eases the joint distribution approximation. The shape feature diffusion facilitates natural object placements, including symmetries. Our method enables many downstream applications, including scene completion, scene arrangement, and text-conditioned scene synthesis. Experiments on the 3D-FRONT dataset show that our method can synthesize more physically plausible and diverse indoor scenes than state-of-the-art methods. Extensive ablation studies verify the effectiveness of our design choice in scene diffusion models.

==> figs/arrangement_supple.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.14\textwidth}
            \includegraphics[width=\textwidth]{./figs/experiments/arrangement_supple/noisy/LivingDiningRoom-270_12_012.jpg}
            \includegraphics[width=\textwidth]{./figs/experiments/arrangement_supple/noisy/LivingDiningRoom-13177_88_442.jpg}
            \includegraphics[width=\textwidth]{./figs/experiments/arrangement_supple/noisy/LivingDiningRoom-64631_169_700.jpg}
            \includegraphics[width=\textwidth]{./figs/experiments/arrangement_supple/noisy/LivingDiningRoom-79295_184_184.jpg}
        \caption{Noisy Scenes}
	\end{subfigure}
        \rulesep
        %%%%
        \begin{subfigure}[t]{0.41\textwidth}
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-270_12_012.jpg}%
            \hfill
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-270_12_204.jpg}%
            \hfill
      	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-270_12_396.jpg} 
            %%%%%%%%%%%%%%%%%%%%%%%
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-13177_88_088.jpg}%
            \hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-13177_88_796.jpg}%
    	\hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-13177_88_973.jpg}
               %%%%%%%%%%%%%%%%%%%%%%%
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-64631_169_523.jpg}%
            \hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-64631_169_700.jpg}%
    	\hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-64631_169_877.jpg}
            %%%%%%%%%%%%%%%%%%%%%%%
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-79295_184_184.jpg}%
            \hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-79295_184_376.jpg}%
    	\hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/atiss/LivingDiningRoom-79295_184_568.jpg}
        \caption{ATISS~\cite{paschalidou2021atiss}}
	\end{subfigure}
        \rulesep
        %%%
	\begin{subfigure}[t]{0.41\textwidth}
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-270_12_014.jpg}
            \hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-270_12_017.jpg}%
    	\hfill
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-270_12_020.jpg}
      %%%%%%%%%%%%%%%%%%%%%%%
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-13177_88_005.jpg}%
            \hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-13177_88_021.jpg}%
    	\hfill
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-13177_88_796.jpg}
      %%%%%%%%%%%%%%%%%%%%%%%
      \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-64631_169_017.jpg}%
            \hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-64631_169_169.jpg}%
    	\hfill
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-64631_169_346.jpg}
           %%%%%%%%%%%%%%%%%%%%%%%
      \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-79295_184_018.jpg}%
            \hfill
            \includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-79295_184_006.jpg}%
    	\hfill
    	\includegraphics[width=0.33\textwidth]{./figs/experiments/arrangement_supple/ours/LivingDiningRoom-79295_184_017.jpg}
		\caption{Ours}
	\end{subfigure}
	\caption{Scene re-arrangements of collections of random objects.  Compared to ATISS, our method generates various object placement options
        with better plausibility.}
    \label{fig:arrangement_supple}
    %\vspace{-4mm}
\end{figure*}


==> figs/uncond_comparison.tex <==
\begin{figure*}[!ht]
	\centering
 	\begin{subfigure}[t]{0.23\textwidth}
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/bed/083_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/bed/134_scene.jpg}
  		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/bed/176_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/bed/404_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/dining/005_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/dining/006_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/dining/052_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/dining/161_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/living/001_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/living/110_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/living/152_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/depthGAN/living/180_scene.jpg}
		\caption{DepthGAN~\cite{yang2021indoor}}
	\end{subfigure}
	\rulesep
	\begin{subfigure}[t]{0.23\textwidth}
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/bed/005_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/bed/042_scene.jpg}
  		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/bed/049_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/bed/067_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/dining/024_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/dining/043_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/dining/078_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/dining/978_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/living/000_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/living/006_scene.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/living/088_scene.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/sync2gen/living/047_scene.jpg}
		\caption{Sync2Gen~\cite{yang2021scene}}
	\end{subfigure}
	\rulesep
        \begin{subfigure}[t]{0.23\textwidth}
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/bed/Bedroom-691_85_234.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/bed/Bedroom-5215_101_850.jpg}
  		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/bed/Bedroom-11202_83_524.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/bed/Bedroom-47437_39_531.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/dining/DiningRoom-164_131_676.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/dining/DiningRoom-2432_86_381.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/dining/DiningRoom-2817_15_455.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/dining/DiningRoom-2817_15_792.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/living/LivingDiningRoom-270_12_095.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/living/LivingDiningRoom-1419_47_031.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/living/LivingDiningRoom-9530_100_053.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/atiss/living/LivingRoom-1097_67_061.jpg}
		\caption{ATISS~\cite{paschalidou2021atiss}}
	\end{subfigure}
	\rulesep
	\begin{subfigure}[t]{0.23\textwidth}
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/bed/Bedroom-2719_8_130.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/bed/Bedroom-22570_139_160.jpg}
  		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/bed/MasterBedroom-19531_93_061.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/bed/SecondBedroom-35274_130_141.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/dining/DiningRoom-164_131_119.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/dining/DiningRoom-12376_156_049.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/dining/DiningRoom-9982_116_095.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/dining/DiningRoom-15534_1_169.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/living/LivingDiningRoom-1625_110_034.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/living/LivingDiningRoom-14432_148_037.jpg}
            \includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/living/LivingDiningRoom-34678_2_215.jpg}%
		\hfill
		\includegraphics[width=0.49\textwidth]
		{figs/experiments/unconditional/ours/living/LivingRoom-3540_79_071.jpg}
		\caption{Ours}
	\end{subfigure}
	\caption{Unconditional scene synthesis. \jiapeng{We compare our method with the state-of-the-art by generating from random noises, where our results present higher diversity and better plausibility with fewer penetration issues.}}
\label{fig:uncond_comparison}
%\vspace{2mm}
\end{figure*}


==> tabs/ablation.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[!htbp]
    % \captionsetup[table]{
    % %labelfont=bf,
    % %textfont=normalfont,
    % textfont=bf,
    % singlelinecheck=off,
    % %justification=raggedright
    % }
	\renewcommand\arraystretch{1.2}
	\begin{center}
		\begin{tabular}{*{5}{c}}
			\toprule
			%\multirow{2}*{Method} & \multicolumn{4}{c}{Bedroom} \\ \cmidrule(lr){2-5}
                Method & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$  & CKL $\downarrow$ \\ % $\times100$ 
			\midrule
			\midrule
            % Ours-Grid-$8^3$
            %       & 31.28  & 14.81 & 84.55  & 6.23 \\

            % Ours-Plane-$32^2$
            %       & 28.17  & 11.12  & 83.80  & 2.67 \\
        
            Ours-PVCNN 
                  & 25.81  & 8.55 & 72.98  & 1.53 \\
                  
            % Ours-Transformer
            %       &   &  &   &  0.17\\

            %Causal 
            Ours-Transformer
                  & 29.08  & 4.59 & 73.63  & 0.36\\

            % Ours-Auto. diff.
            %       &   &  &   & \\

            Ours-Single head
                    & 19.78  & 2.07 & 54.53  & 0.69 \\

            Ours-w/o pos. emb. 
                    &   &   &   & \\ 
            Ours-w/o iou reg. 
                    &   &   &   & \\
                    
            Ours-w/o geometry code  
                   & 18.40  & 1.55  & 55.42 & 0.66 \\

            Ours-final
                   & \textbf{18.29} & \textbf{1.42}  & \textbf{53.52}  & \textbf{0.35}  \\

        \bottomrule
        \end{tabular}
        \caption{Quantitative ablation studies on the task of unconditional scene synthesis on the 3D-FRONT bedrooms.} % Note that for the Scene Classification Accuracy (SCA), the score close to 0.5 is better.
        \label{tab:ablation}
        \end{center}
        \vspace{-6mm}
\end{table}

==> tabs/arrangement.tex <==
\setlength{\tabcolsep}{2.4pt}
\begin{table}[!hbt]
    % \captionsetup[table]{
    % %labelfont=bf,
    % %textfont=normalfont,
    % textfont=bf,
    % singlelinecheck=off,
    % %justification=raggedright
    % }
	%\renewcommand\arraystretch{1.2}
         %\setlength{\tabcolsep}{1.5pt}
         \footnotesize
	\begin{center}
		\begin{tabular}{*{11}{c}}
			\toprule
			\multirow{2}*{Method} & \multicolumn{5}{c}{Dining room}   & \multicolumn{5}{c}{Living room} \\
			\cmidrule(lr){2-6} \cmidrule(lr){7-11}
			 & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$   & \#Sym. & IoU   & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$  & \#Sym. & IoU  \\
			\midrule
			\midrule
            ATISS
                  & 43.40   & 7.85 & 63.99  & &
                  & 43.98  & 6.73 & 73.83 & & \\

            LEGO-Net
                 &  &   &  & &
                %& LEGO-Net & 48.49  & 7.79  & 77.34 \\
                 & 45.40  & 9.57  & 82.03 & & \\
            
            Ours
                  &\textbf{40.84} & \textbf{2.21} & \textbf{40.36} & &%-54k
                  & \textbf{42.92} & \textbf{2.81}  & \textbf{61.13} & & \\ % -99k \\

        \bottomrule
        \end{tabular}
        \caption{Quantitative comparisons on the task of \textbf{scene arrangement} on the 3D-FRONT bedrooms and dining rooms. Given a collection of objects as inputs, we predict their locations and orientations to obtain object placements.}
        \label{tab:arrange}
        \end{center}
        \vspace{-6mm}
\end{table}

==> tabs/completion.tex <==
\setlength{\tabcolsep}{2.4pt}
\begin{table}[!hbt]
    % \captionsetup[table]{
    % %labelfont=bf,
    % %textfont=normalfont,
    % textfont=bf,
    % singlelinecheck=off,
    % %justification=raggedright
    % }
    \renewcommand\arraystretch{1.2}
    \begin{center}
        \begin{tabular}{*{6}{c}}
            \toprule
            \multirow{2}*{Method} \cmidrule(lr){2-6} 
             & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$  & Sym. &  PIoU \\
            \midrule
            \midrule
            ATISS~\cite{paschalidou2021atiss}
                  & 30.54  & 2.38 & 26.73  & &
                  & 42.65  & 8.32 & 43.99  & &\\
            
            Ours
                 & \textbf{27.32} & \textbf{1.92}  & \textbf{40.30} 
                   & \textbf{40.99} & \textbf{6.31}  & \textbf{49.06}  \\
        \bottomrule
        \end{tabular}
        \caption{Quantitative comparisons on the task of scene completion on the 3D-FRONT bedrooms and dining rooms. Only 3 objects are given in the partial scenes. }
        \label{tab:completion}
        \end{center}
        \vspace{-6mm}
\end{table}


==> tabs/text.tex <==
% %\setlength{\tabcolsep}{4pt}
% \begin{table}[h]
%     % \captionsetup[table]{
%     % %labelfont=bf,
%     % %textfont=normalfont,
%     % textfont=bf,
%     % singlelinecheck=off,
%     % %justification=raggedright
%     % }
% 	\renewcommand\arraystretch{1.2}
% 	\begin{center}
% 		\begin{tabular}{*{7}{c}}
% 			\toprule
% 			\multirow{2}*{Method} & \multicolumn{3}{c}{Bedroom}   & \multicolumn{3}{c}{Dining room} \\
% 			\cmidrule(lr){2-4} \cmidrule(lr){5-7}
% 			 & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$   & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$
%      \\ % $\times100$ 
% 			\midrule
% 			\midrule
%             ATISS
%                   & 19.01  & 1.84 &  59.00
%                   & 36.61  & 1.90 & 55.44  \\
            
%             Ours
%                   & \textbf{18.52} & \textbf{1.58}  & \textbf{53.23} 
%                   & \textbf{32.87} & \textbf{0.57}  & \textbf{51.67}  \\
%         \bottomrule
%         \end{tabular}
%         \caption{Quantitative comparisons on the task of \textbf{text-conditioned scene synthesis} on the 3D-FRONT bedrooms and dining rooms. }
%         \label{tab:text}
%         \end{center}
%         %\vspace{-10mm}
% \end{table}


\setlength{\tabcolsep}{2.4pt}
\begin{table}[h]
    % \captionsetup[table]{
    % %labelfont=bf,
    % %textfont=normalfont,
    % textfont=bf,
    % singlelinecheck=off,
    % %justification=raggedright
    % }
	\renewcommand\arraystretch{1.2}
	\begin{center}
		\begin{tabular}{*{7}{c}}
			\toprule
			\multirow{2}*{Method} & \multicolumn{3}{c}{Dining room}   & \multicolumn{3}{c}{Living room} \\
			\cmidrule(lr){2-4} \cmidrule(lr){5-7}
			 & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$   & FID $\downarrow$ & KID $\downarrow$ & SCA $\%$
     \\ % $\times100$ 
			\midrule
			\midrule
            ATISS
                   & 36.61  & 1.90 & 55.44  
                   & 40.45  & 4.57 & 63.48 \\
            
            Ours
                  & \textbf{32.87} & \textbf{0.57}  & \textbf{51.67} 
                  & \textbf{35.27} & \textbf{0.64}  & \textbf{54.69}  \\
        \bottomrule
        \end{tabular}
        \caption{Quantitative comparisons on the task of \textbf{text-conditioned scene synthesis} on the 3D-FRONT dining and living rooms. }
        \label{tab:text}
        \end{center}
        %]\vspace{-10mm}
\end{table}


==> tabs/text_user.tex <==


%\setlength{\tabcolsep}{4pt}
\begin{table}[h]
    % \captionsetup[table]{
    % %labelfont=bf,
    % %textfont=normalfont,
    % textfont=bf,
    % singlelinecheck=off,
    % %justification=raggedright
    % }
	\renewcommand\arraystretch{1.2}
	\begin{center}
		\begin{tabular}{*{5}{c}}
			\toprule
			\multirow{2}*{Method} & \multicolumn{2}{c}{Bedroom}   & \multicolumn{2}{c}{Dining room} \\
			\cmidrule(lr){2-3} \cmidrule(lr){4-5}
			 & match & realism    & match & realism
     \\ % $\times100$ 
			\midrule
			\midrule
            ATISS
                  &   &   
                  &   &   \\
            
            Ours
                 & \textbf{} & \textbf{} 
                   & \textbf{}  & \textbf{}  \\
        \bottomrule
        \end{tabular}
        \caption{Perceptual use study of \textbf{text-conditioned scene synthesis} on the 3D-FRONT bedrooms and dining rooms. }
        \label{tab:text_user}
        \end{center}
        %\vspace{-10mm}
\end{table}
